LLMigrate: Transforming "Lazy" Large Language Models into Efficient Source Code Migrators

Rewriting C code in Rust provides stronger memory safety, yet migrating large codebases such as the 32-million-line Linux kernel remains challenging. While rule-based translators (e.g., C2Rust) provide accurate yet largely unsafe Rust programs, recent Large Language Model (LLM) approaches produce more idiomatic, safe Rust programs but frequently exhibit "laziness", omitting significant portions of the target code. To address the issue, in this paper, we present LLMigrate, an LLM-based C-to-Rust translation tool that splits modules into discrete functions, translating them individually, and then reintegrating them. LLMigrate uses static analysis to retain necessary context, pairs GPT-4o (a state-of-the-art LLM) with compiler-driven translation and program-repair techniques for complex core functions, and leverages call-graph-guided translation to ensure consistent interfaces. Evaluations on three representative Linux kernel modules (math, sort, and ramfs) show that LLMigrate requires modifying less than 15\% of the target code, significantly outperforming a pure GPT-4o-based migration.

==> tables/fun-repair.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \begin{tabular}{|c|c|cc|cc|}
% \hline
% {\color[HTML]{333333} } &
%   {\color[HTML]{333333} } &
%   \multicolumn{2}{c|}{{\color[HTML]{333333} \# MML}} &
%   \multicolumn{2}{c|}{{\color[HTML]{333333} \% MML}} \\ \cline{3-6} 
% \multirow{-2}{*}{{\color[HTML]{333333} Dataset}} &
%   \multirow{-2}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\# Modified\\ functions\end{tabular}}} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} mean}} &
%   {\color[HTML]{333333} std} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} mean}} &
%   {\color[HTML]{333333} std} \\ \hline
% {\color[HTML]{333333} lz4} &
%   {\color[HTML]{333333} 18/60} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 8.44}} &
%   {\color[HTML]{333333} 7.08} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 10.25\%}} &
%   {\color[HTML]{333333} 8.1\%} \\ \hline
% {\color[HTML]{333333} sort} &
%   {\color[HTML]{333333} 6/12} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 5}} &
%   {\color[HTML]{333333} 2.45} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 10.59\%}} &
%   {\color[HTML]{333333} 7.5\%} \\ \hline
% {\color[HTML]{333333} ramfs} &
%   {\color[HTML]{333333} 21/21} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 8.8}} &
%   {\color[HTML]{333333} 8.52} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 0.20\%}} &
%   {\color[HTML]{333333} 0.17\%} \\ \hline
% \end{tabular}
% \caption{The number (\#) and proportion (\%) of Manually Modified Lines (MMLs) required to achieve successful compilation during the function-level repair stage. We calculate the mean and standard deviation of MMLs across all modified functions for each dataset.}
% \label{tab:fun-repair}
% \end{table}

==> tables/repair.tex <==


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \begin{tabular}{|c|cc|cc|cc|}
% \hline
% {\color[HTML]{333333} } &
%   \multicolumn{2}{c|}{{\color[HTML]{333333} Mod}} &
%   \multicolumn{2}{c|}{{\color[HTML]{333333} Repo}} &
%   \multicolumn{2}{c|}{fun+mod+repo} \\ \cline{2-7} 
% \multirow{-2}{*}{{\color[HTML]{333333} Dataset}} &
%   \multicolumn{1}{c|}{\#} &
%   \% &
%   \multicolumn{1}{c|}{\#} &
%   \% &
%   \multicolumn{1}{c|}{\#} &
%   \% \\ \hline
% {\color[HTML]{333333} lz4} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 32}} &
%   0.95\% &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 46}} &
%   1.36\% &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 230}} &
%   {\color[HTML]{333333} 6.79\%} \\ \hline
% {\color[HTML]{333333} sort} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 8}} &
%   0.19\% &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 8}} &
%   0.19\% &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 46}} &
%   {\color[HTML]{333333} 14.33\%} \\ \hline
% {\color[HTML]{333333} ramfs} &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 14}} &
%   0.24\% &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 77}} &
%   1.33\% &
%   \multicolumn{1}{c|}{{\color[HTML]{333333} 227}} &
%   {\color[HTML]{333333} 4.77\%} \\ \hline
% \end{tabular}
% \caption{The number (\#) and proportion (\%) of Manually Modified Lines (MMLs) required to achieve successful compilation during the module-level repair stage, the repo-level repair stage, and the total MMLs of the three stages (function level, module level, and repo level).}
% \label{tab:repair}
% \end{table}

==> tables/sub_datasets.tex <==


% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% {\color[HTML]{333333} Dataset} &
%   {\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\# Funs\end{tabular}} &
%   {\color[HTML]{333333} \# Lines} &
%   {\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\# Extern\\ vars\end{tabular}} &
%   {\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\# Extern\\ funs\end{tabular}} &
%       {\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\# Intern\\ funs\end{tabular}} \\ \hline
% {\color[HTML]{333333} lz4} &
%   {\color[HTML]{333333} 6} &
%   {\color[HTML]{333333} 114} &
%   {\color[HTML]{333333} 24} &
%   {\color[HTML]{333333} 7} &
%   {\color[HTML]{333333} 4} \\ \hline
% {\color[HTML]{333333} sort} &
%   {\color[HTML]{333333} 6} &
%   {\color[HTML]{333333} 66} &
%   {\color[HTML]{333333} 7} &
%   {\color[HTML]{333333} 0} &
%   {\color[HTML]{333333} 0} \\ \hline
% {\color[HTML]{333333} ramfs} &
%   {\color[HTML]{333333} 6} &
%   {\color[HTML]{333333} 334} &
%   {\color[HTML]{333333} 36} &
%   {\color[HTML]{333333} 38} &
%   {\color[HTML]{333333} 4} \\ \hline
% \end{tabular}
% \caption{Statistics of datasets. Each dataset is a subset of the datasets shown in Table 1, with a varying number of functions, lines of code, external variables, external functions, and internal function calls.}
% \label{tab:sub_datasets}
% \end{table}
